RABBiT: Rapidly adaptive BOLD foundation model via brain-tuning for accurate zero-shot and few-shot prediction of speech-elicited responses in the brain

Language understanding in the brain is context-dependent, varying across experimental stimuli and individuals, which makes it difficult to build computational models that generalize across both. This calls for a foundation model of language-evoked brain activity that can capture shared structure while adapting efficiently to new participants and inputs. We introduce RABBiT (Rapidly Adaptive BOLD foundation model via BraIn-Tuning), a compact audio-to-fMRI encoder designed for accurate zero- and few-shot prediction. A comprehensive evaluation on 324 participants across multiple unseen fMRI datasets shows that RABBiT enables accurate zero-shot prediction of fMRI responses to natural speech across auditory and language-selective regions, surpassing the SOTA foundation model for fMRI and predictions based on group averages. With as little as 10 minutes of participant-specific data, RABBiT further improves performance via parameter-efficient tuning, substantially outperforming per-participant linear models. RABBiT's performance is driven by two key innovations: (1) learned region-specific attention, and (2) a decomposition of brain responses into shared and subject-specific components, combined with a brain-tuned speech backbone. In addition to supporting strong predictive accuracy, the structured, region-specific representations that RABBiT learns enable interpretability. By eliminating the need for extensive per-participant data and model fitting, RABBiT enables scalable population-level analyses of language in the human brain. We make the code available at https://github.com/bridge-ai-neuro/rabbit.

==> 1-abstract_intro_old.tex <==

\begin{abstract}

Language understanding in the brain is context-dependent, varying across experimental stimuli and individuals, which makes it difficult to build computational models that generalize across both. This calls for a foundation model of language-evoked brain activity that can capture shared structure while adapting efficiently to new participants and inputs. We introduce RABBiT (Rapidly Adaptive BOLD foundation model via BraIn-Tuning), a compact audio-to-fMRI encoder designed to meet this need. A comprehensive evaluation on 324 participants across multiple unseen fMRI datasets shows that RABBiT enables accurate zero-shot prediction of fMRI responses to natural speech across auditory and language-selective regions, surpassing the SOTA foundation model for fMRI and predictions based on group averages. With as little as 10 minutes of participant-specific data, RABBiT further improves performance via parameter-efficient tuning, substantially outperforming per-participant linear models. In addition to strong predictive accuracy, RABBiT learns structured, region-specific representations that reflect the cortical hierarchy of language processing. By eliminating the need for extensive per-participant data and model fitting, RABBiT enables scalable population-level analyses of language in the human brain.

%Language is uniquely human, distributed across cortex, and idiosyncratic across people, making it the least understood of high cognitive functions. Without a model organism to study language, researchers tried to understand it from fMRI data with encoding models that fit per-subject linear ridge encoders which fail at  predicting accurate response to an unseen spoken stimulus without the need for recording fMRI data. Other recent approaches train large multi-modal encoders that can predict whole-brain responses, but they don't predict high-resolution language responses, and they can't be adapted easily to fit new subjects with small data. Hence, there is a strong need for a \textbf{foundation model of language-evoked fMRI}: one encoder that does exactly that, accurately and across all language-relevant regions while enabling easy and cheap adaptation to new subjects.

%We introduce \textbf{RABBiT} (Rapidly Adaptive BOLD foundation model via BraIn-Tuning), a compact audio-to-fMRI encoder designed around this goal. Trained on 6 participants and evaluated on \textbf{324 unseen participants} across different fMRI studies, RABBiT’s zero-shot \textit{exceeds the inter-subject noise ceiling} and the state-of-the-art multi-subject encoders across auditory and language ROIs. It also enables Few-shot prediction; after $\sim$ 10 min of calibration on a new subject, it improves over zero-shot and significantly outperforms per-subject linear ridge regression while needing \textbf{3 orders of magnitude} less parameters. Finally, RABBiT learns per-ROI query embeddings that mirror the cortical hierarchy of language in the brain. By removing the per-subject scanning and ridge fit between the model and any new subject, RABBiT opens fast and accurate population-level analyses of language processing in the brain.
% Self-supervised speech models align with human brain responses during
% naturalistic listening, making them fit as organisms for studying
% language processing in the brain. Fine-tuning these models directly on fMRI --- \emph{brain-tuning} ---
% has been shown to improve alignment further and reduces per-subject data cost. Yet, previous brain-tuned encoders were not designed for zero-shot or few-shot settings; they require a participant-specific voxel-wise encoding head
% from each new participant, which scales linearly
% with cohort size, and limits population-level analyses. Recent multimodal
% encoders (e.g.\ TRIBEv2, \citealp{dAscoli2026TribeV2}) scale across participants by combining frozen
% foundational backbones with per-subject output projections and large ensembles, but they scale poorly to large number of participants, predict low-resolution cortical surfaces, perform poorly on primary sensory regions, and are costly to run and train.

% We introduce \textbf{PEBT} (Parameter Efficient Brain-tuning Transformer), a
% lightweight audio-to-fMRI encoder that supports zero-shot and
% parameter-efficient few-shot prediction across $\sim$41K cortical voxels in auditory and language regions (4x the resolution of the state of the art). PEBT uses
% brain-tuning with a novel cross-attention temporal transformer, and a low-rank shared$+$deviation decomposition of each ROI's
% response that are trained to capture both shared responses and idiosyncrasies well.

% Trained on 6 participants and evaluated on 156 unseen participants across 8
% held-out English naturalistic stories, PEBT achieves the following: (i) Zero-shot exceeds the state-of-the-art multi-modal brain encoder and the inter-subject noise ceiling in auditory and language
% regions, (ii) Being designed for efficient few-shot calibration, PEBT beats standard linear per-participant linear encoding with only $\sim$10 minutes of data, using two orders of magnitude fewer parameters; and (iii)  Learned per-ROI attention weights also align with the cortical hierarchy of temporal integration timescales.
% Together, these findings reframe brain-tuning as a route to lightweight,
% transferable brain encoders for population-level analyses of speech and
% language processing.
\end{abstract}

% =====================================================================
\section{Introduction}
\label{sec:intro}

Self-supervised speech and language models align with human brain responses
elicited by naturalistic stimuli
\citep{toneva2019interpreting,schrimpf2021neural,goldstein2022shared,oota2024speech},
and this alignment can be further improved by directly fine-tuning the
model on fMRI --- an approach known as \emph{brain-tuning}. Initial work
demonstrated this on a single participant at a time, both as a way to make
the resulting speech representations more useful for downstream semantic
tasks \citep{moussa2025improving} and as a way to improve voxel-wise brain
prediction in the same listener \citep{vattikonda2025brainwavlm}.
\citet{moussa2025multibrain} subsequently extended brain-tuning to multiple
participants jointly, reducing the data needed to align an encoder to a
new participant by $\sim$5$\times$, improving alignment by up to
$\sim$50\%, and producing speech backbones that transfer to downstream
semantic tasks even on listeners unseen at training.

However, brain-tuning was never adopted to zero-shot and few-shot settings: every prediction in a new participant requires a voxel-wise linear readout fit on fresh fMRI from that participant. This blocks zero-shot evaluation
of the encoder, scales linearly with cohort size, and limits
population-level analyses. Concurrent multimodal encoders take a different
route: TRIBEv2 \citep{dAscoli2026TribeV2} and universal brain encoders
\citep{beliy2025brainlm} scale across many participants by combining frozen
pretrained foundation backbones with per-subject output projections and
large model ensembles (TRIBEv2 is 1B parameters \citep{dAscoli2026TribeV2}). They reach high accuracy on group-level metrics, but but they are expensive to train on many subjects (scale linearly because of independent subject heads), they predict low-resolution cortical surfaces, perform poorly on primary sensory regions, and are costly to run and train. Per-subject ridge regression
\citep{huth2016natural} remains a strong individual baseline but offers no
transfer and is data hungry \citep{antonello2024scaling}.
We address these limitations with \textbf{RABBiT} (Rapidly Adaptive BOLD foundation model via BraIn-Tuning; Fig.\ref{fig:overview}), a lightweight brain-tuned
audio-to-fMRI encoder that supports both zero-shot and parameter-efficient
few-shot prediction of brain responses in new participants from a single
trained model. RABBiT combines three components. The first is a
parameter-efficient brain-tuning of a self-supervised speech backbone
(e.g., Wav2Vec2.0\citep{baevski2020wav2vec}) The second is a small temporal brain transformer that replaces the standard voxel-wise linear readout with a brain transformer, with anatomical ROI query tokens ( from HCP-MMP1; \citep{glasser2016multi}). The transformer learns to route speech features to brain regions, turning the readout into interpretable per-region predictions rather than millions of voxel-wise ridge weights. The third is a low-rank brain decomposition of each ROI's response --- a learnable population-shared projection and a small per-subject deviation from the mean. This enables both transfer regimes efficiently: for zero-shot, the model predicts the expectation of the learned projections as the group-level response, and for few-shot, this low-rank projection can be tuned with few minutes of subject data.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.40\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/teaser-branching.pdf}
    \caption{PEBT transfers after training.}
    \label{fig:teaser}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.58\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/transformer.pdf}
    \caption{Cross-attention module in brain transformer.}
    \label{fig:trans}
  \end{subfigure}\\[6pt]
  \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/training-process.pdf}
    \caption{Training: predict fMRI per ROI, compare to measured.}
    \label{fig:training}
  \end{subfigure}
  \caption{\textbf{Overview of RABBiT.}
    \textbf{(a)}~A single encoder that supports two
    transfer regimes for new subjects. \emph{Zero-shot}: predicting group-level responses; tested on 324 unseen participants across 16 held-out studies with naturalistic listening; RABBiT's predictions on auditory ROIs already saturate near the inter-subject ceiling. \emph{Few-shot}: adapting to a new subject with small data;  RABBiT rapidly and effectively adapts to unseen subjects with only $\sim$10 minutes of paired audio, improving mostly idiosyncratic language ROIs with 3 order of magnitude less paramters than voxel-wise models. \textbf{(b)}~The cross-attention readout: learnable ROI query tokens attend to audio output tokens of the speech backbone, yielding a per-ROI latent $z_i$ that feeds to prediction heads. The highlighted query (\emph{IFG}) illustrates the $W_Q,W_K,W_V$ / softmax / weighted-sum path; the heatmap shows the resulting attention weights. \textbf{(c)}~Training pipeline. Audio is encoded by a speech model into a temporal token sequence; the cross-attention transformer routes those tokens to ROI latents; the per ROI latent passes through our low-rank decomposition(learnable shared + per-subject Idiosyncratic components) to form the predicted fMRI response; the loss is applied between predicted and measured fMRI. The whole pipeline has $\approx$12.4M trainable parameters.}
  \label{fig:overview}
\end{figure}

PEBT is trained on only 6 participants from the Friends dataset \citep{boyle2025friends}) and is then able to strongly predict group-level brain responses to new stimuli ( tested against 324 unseen participants across 16 held-out studies). It can also improve subject-specific responses for any new subject after a brief $\sim$10-minute calibration session (i.e., a few-shot regime). At zero-shot, PEBT exceeds the inter-subject noise ceiling in language regions and the multimodal TRIBEv2 baseline \citep{dAscoli2026TribeV2}. At few-shot calibration, it exceeds per-subject ridge regression performance with roughly two orders of magnitude fewer parameters, with the largest gains in higher-order language regions that are most idiosyncratic across subjects.

To summarize, our main contributions are:
\begin{itemize}
  \item[(i)] We present a \textbf{lightweight, brain-tuned audio-to-fMRI
        encoder} that supports both zero-shot and parameter-efficient
        few-shot prediction of speech-elicited fMRI in new listeners
        without participant-specific readout fitting, establishing
        brain-tuning as a transferable tool.
  \item[(ii)] On 324 unseen participants across 16 naturalistic stories, RABBiT exceeds TRIBEv2 \citep{dAscoli2026TribeV2} and the inter-subject noise ceiling at zero-shot prediction.
  \item[(iii)] We beat per-subject ridge regression at few-shot in higher-order language regions, with two orders of magnitude fewer parameters.
  \item[(iv)] Learnable query attention:
        per-ROI attention weights align with the cortical hierarchy of temporal integration timescales, providing a readout of how the model routes speech features to brain regions.
\end{itemize}


==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the abstract and at the end of the introduction and results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:\answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In section 5, this is discussed explicitly.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Our framework is mainly empirical and does not involve formal proofs or theoretical assumptions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We describe in the Methods section and throughout the Appendix the details and analyses of the experimental setups for all experiments and design choices.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our code and trained models will be released publicly; as for the datasets used, they are publicly available datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer:  \answerYes{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Evaluation setup, experimental details, and hyperparameters are details in the methods and appendices.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:\answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Throughout all quantitative results, we provide error bars and carry out statistical significance tests; details for each test performed are in the Results section and appendices. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Methods and appendix C has all details regarding computer resources, training times, and so on to replicate the results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Going through the code of ethics, we are convinced that we have complied with NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the discussion, we have addressed the broader impacts of our work, and related things around that. Moreover, our research is mainly scientific exploration and doesn't pose additional social risks. That is why we have not included detailed discussions on potential harmfulness.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper and methods poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use public fMRI datasets, and whenever required asked the original dataset authors for access/metadata. We also rely on open source pretrained speech models. Use of datasets and models are properly credited and cited in the paper with all details on where and how they are obtained and used.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Upon publication, our code and trained models will be released publicly with proper documentation; it will be documented such that it's easy to use by others.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer:\answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All used datasets were publicly available and collected by others.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}  % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The data we use is public and previously collected by others.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: pretrained speech models are used through the paper. We describe their usage in the methods and appendices. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}
